Grammatical Error Correction in Low Error Density Domains: A New Benchmark and Analyses

Evaluation of grammatical error correction (GEC) systems has primarily focused on essays written by non-native learners of English, which however is only part of the full spectrum of GEC applications. We aim to broaden the target domain of GEC and release CWEB, a new benchmark for GEC consisting of website text generated by English speakers of varying levels of proficiency. Website data is a common and important domain that contains far fewer grammatical errors than learner essays, which we show presents a challenge to state-of-the-art GEC systems. We demonstrate that a factor behind this is the inability of systems to rely on a strong internal language model in low error density domains. We hope this work shall facilitate the development of open-domain GEC models that generalize to different topics and genres.

==> figures/corpora_stats.tex <==
\begin{table*}[th]
    \centering
    \begin{small}
    \begin{tabular}{lrccccccccc}
        \toprule
         & \textbf{\# sents} & \textbf{type-token} & \textbf{tok/sent} & \textbf{err. sents} (\%) & \textbf{edits/sent} & \textbf{\# annotators} & \textbf{sent-$\mathcal{K}$} & \textbf{NEs/sents}  \\
        \midrule
        JFLEG & 747 & 0.44 & 18.9 & 95.7 & 3.6 & 4 & 0.53 & 0.35 \\
        \midrule
        %FCE & 2,710 & 0.39 & 15.5 & 65.9 & 2.5 & - & - & 0.59 \\
        FCE 2.1 & 2,695 & 0.39  & 15.6 & 67.8 & 2.6 & 1 & - & 0.59 \\
        \midrule
        CoNLL14 & 1,312 & 0.4 & 22.9 & 89.6 & 2.4 & 2 & 0.25 & 0.50 \\
        \midrule
        W\&I-A & 1,036 & 0.43 & 18.0 & 79.1 & 3.6 & 1 & - & 0.58 \\
        W\&I-B & 1,285 & 0.45 & 18.4 & 71.6 & 2.7 & 1 & - & 0.52 \\
        W\&I-C & 1,068 & 0.47 & 20.1 & 53.5 & 1.9 & 1 & - & 0.78 \\
        \midrule
        LOCNESS & 988 & 0.47 & 23.4 & 51.3 & 1.8 & 1 & - & 0.77 \\
        \midrule
        GMEG wiki & 992 & 0.55 & 26.9 & 95.5 & 2.5 & 4 & 0.43 & 2.84 \\
        GMEG yahoo & 1,000 & 0.46 & 16.9 & 71.8 & 2.7 & 4 & 0.51 & 0.60 \\
        \midrule
        AESW & 52,124 & 0.52 & 23.9 & 36.1 & 1.6  & 1 & - & 0.93 \\
        \midrule
        CWEB-S & 2,864 & 0.56 & 23.9 & 35.9 & 1.5 & 2 & 0.39 & 1.43 \\
        CWEB-G & 3,981 & 0.53 & 20.3 & 36.3 & 1.9 & 2 & 0.44 & 1.03 \\
        \bottomrule
    \end{tabular}
    \end{small}
    \caption{Statistics on GEC Corpora; type--token is the average ratio of vocabulary size by the total number of tokens (calculated as an average over a sliding window of $1,000$ tokens); a sentence is erroneous if at least one annotator made an edit; ratio of edits per sentence is calculated on erroneous sentences; $\mathcal{K}$ is Cohen's Kappa score (sentence level); NEs stands for Named Entities (calculated using Spacy predictions).}
    \label{tab-stats}
\end{table*}

==> figures/sota_scores.tex <==
\begin{table*}[t]
    \centering
    %\begin{small}
    \begin{tabular}{lrcc|ccc}
        \toprule
        & \textbf{P} & \textbf{R} & \textbf{\fhalf}  & \textbf{P} & \textbf{R} & \textbf{\fhalf}  \\
        \midrule
        \midrule
        %\parbox[t]{4mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{SOTA}}}} 
        & \multicolumn{3}{c}{\textsc{\textbf{GEC-pseudodata}}} & \multicolumn{3}{c}{\textsc{\textbf{PIE}}} \\
            \midrule JFLEG & 55.73 & 38.73 & 51.13 & 51.04 & 35.21 & 46.74 \\
            \midrule FCE 2.1 & 55.11 & 41.61 & 51.75 & 49.55 & 36.34 & 46.19 \\
            %FCE & 53.96 & 41.42 & 50.88 & 48.51 & 36.16 & 45.41 \\
            \midrule CoNLL14 & 44.96 & 29.03 & 40.35 & 43.47 & 27.93 & 38.95 \\
            \midrule W\&I-A & 54.89 & 37.92 & 50.38 & 50.24 & 36.1 & 46.59 \\
            W\&I-B & 54.86 & 35.14 & 49.32 & 49.12 & 31.2 & 44.06 \\
            W\&I-C & 44.53 & 32.04 & 41.31 & 39.12 & 27.13 & 35.94 \\
            \midrule
            \midrule
            LOCNESS & 47.09 & 34.13 & 43.77 & 32.77 & 23.11 & 30.24 \\
            \midrule GMEG Wiki & 52.81 & 23.02 & 41.89 & 44.71 & 19.66 & 35.58 \\
            GMEG Yahoo & 37.57 & 32.26 & 36.0 & 33.08 & 26.97 & 31.29 \\
            \midrule AESW & 14.05 & 13.24 & 13.88 & 8.78 & 9.67 & 8.94 \\
            \midrule CWEB-G & 21.34 & 23.0 & 21.58 & 14.29 & 18.91 & 14.98 \\
            CWEB-S & 17.27 & 15.75 & 16.91 & 5.73 & 8.78 & 6.15 \\
            \textbf{{CWEB}} (all) & 19.97 & 20.28 & 19.98 & 10.8 & 15.11 & 11.43 \\
        \bottomrule
    \end{tabular}
    %\end{small}
    \caption{Scores of two \textsc{sota} GEC systems on each domain. Scores are calculated against each individual annotator and averaged in order to be able to compare performance on datasets with different number of annotators.}
    \label{tab-results}
\end{table*}




==> figures/stat_significance.tex <==
\begin{table*}[th]
    \centering
    \begin{tiny}
    \begin{tabular}{lrccccccccccc}
& \textbf{JFLEG} & \textbf{FCE} & \textbf{CoNLL14} & \textbf{W\&I-A} & \textbf{W\&I-B} & \textbf{W\&I-C} & \textbf{LOCNESS} & \textbf{GMEG-Wiki} & \textbf{GMEG-Yahoo} & \textbf{AESW} & \textbf{CWEB-S} & \textbf{CWEB-G}\\
\textbf{\textbf{JFLEG}} & - & 9.4e-19\textbf{*} & 5.8e-63\textbf{*} & 5.6e-14\textbf{*} & 1.1e-39\textbf{*} & 1e-15\textbf{*} & 4.4e-16\textbf{*} & 9.5e-263\textbf{*} & 1.6e-114\textbf{*} & 0\textbf{*} & 2.3e-310\textbf{*} & 7.5e-244\textbf{*}\\
\textbf{\textbf{FCE}} & - & - & 2.9e-12\textbf{*} & 0.41 & 3.1e-08\textbf{*} & 3.3e-16\textbf{*} & 2.3e-15\textbf{*} & 4.3e-15\textbf{*} & 3.1e-38\textbf{*} & 1.2e-292\textbf{*} & 4e-175\textbf{*} & 9.9e-114\textbf{*}\\
\textbf{\textbf{CoNLL14}} & - & - & - & 2e-09\textbf{*} & 0.68 & 1.6e-15\textbf{*} & 2.2e-16\textbf{*} & 5.2e-80\textbf{*} & 6.7e-16\textbf{*} & 2.5e-247\textbf{*} & 4.6e-142\textbf{*} & 4.9e-87\textbf{*}\\
\textbf{\textbf{W\&I-A}} & - & - & - & - & 1.3e-07\textbf{*} & 2.6e-32\textbf{*} & 2.2e-15\textbf{*} & 2.5e-71\textbf{*} & 1.8e-28\textbf{*} & 3.7e-153\textbf{*} & 4.9e-15\textbf{*} & 1e-78\textbf{*}\\
\textbf{\textbf{W\&I-B}} & - & - & - & - & - & 0\textbf{*} & 4e-13\textbf{*} & 4.4e-16\textbf{*} & 5.2e-15\textbf{*} & 6.5e-123\textbf{*} & 5.2e-95\textbf{*} & 1.1e-15\textbf{*}\\
\textbf{\textbf{W\&I-C}} & - & - & - & - & - & - & 0.24 & 5e-06\textbf{*} & 0.00011\textbf{*} & 7.5e-24\textbf{*} & 2.6e-20\textbf{*} & 6.7e-06\textbf{*}\\
\textbf{\textbf{LOCNESS}} & - & - & - & - & - & - & - & 0.012\textbf{*} & 0.0021\textbf{*} & 3.2e-17\textbf{*} & 1.3e-18\textbf{*} & 0.00011\textbf{*}\\
\textbf{\textbf{GMEG-Wiki}} & - & - & - & - & - & - & - & - & 2.9e-15\textbf{*} & 1.1e-43\textbf{*} & 4.9e-27\textbf{*} & 0.0045\textbf{*}\\
\textbf{\textbf{GMEG-Yahoo}} & - & - & - & - & - & - & - & - & - & 1.9e-92\textbf{*} & 2.6e-15\textbf{*} & 8.9e-16\textbf{*}\\
\textbf{\textbf{AESW}} & - & - & - & - & - & - & - & - & - & - & 0.00087\textbf{*} & 8.7e-20\textbf{*}\\
\textbf{\textbf{CWEB-S}} & - & - & - & - & - & - & - & - & - & - & - & 5.2e-16\textbf{*}\\
\textbf{\textbf{CWEB-G}} & - & - & - & - & - & - & - & - & - & - & - & -\\
        \bottomrule
    \end{tabular}
    \end{tiny}
    \caption{TEST}
    \label{tab-stats}
\end{table*}
